LWE-based Identification Schemes

Some hard problems from lattices, like LWE (Learning with Errors), are particularly suitable for application in Cryptography due to the possibility of using worst-case to average-case reductions as evidence of strong security properties. In this work, we show two LWE-based constructions of zero-knowledge identification schemes and discuss their performance and security. We also highlight the design choices that make our solution of both theoretical and practical interest.

==> performance.tex <==
Let us calculate the average communication costs for this identification scheme. Whenever a random vector is supposed to be exchanged between the Prover and the Verifier, we send the corresponding seed from which the element can be obtained, assuming that both parties agree upon the use of a pseudo-random generator. The definition of the isometry $\Pi_{\vector{\gamma,\Sigma}}$ takes two seeds (one for vector $\vector{\gamma}$ and one for permutation $\Sigma$). The number of bits of a given element is returned by the application of $\left|seed\right|$.  Therefore, the payload breakdown per round of execution can be seen as follows:
\begin{itemize}
 \item Commitments: $3\left|com\right|$;
 \item Challenge: $\left\lceil \log_2{\text{max}(ch)} \right\rceil$;
 \item Answer: $\frac{10}{3}\left|seed\right|+\frac{2}{3}(m+n)\left\lceil \log_2{q}\right\rceil$, which is the average of 
 \begin{itemize}
	\item for $ch=1$: $4\left|seed\right|+m\left\lceil \log_2{q}\right\rceil$;
	\item for $ch=2$: $2\left|seed\right|+2n\left\lceil \log_2{q}\right\rceil$;
	\item for $ch=3$: $4\left|seed\right|+m\left\lceil \log_2{q}\right\rceil$.
 \end{itemize}
\end{itemize}


==> security.tex <==
There are two security aspects to be taken into account regarding the scheme: the hardness of the underlying LWE problem and the overall soundness error.
The first factor is linked with the values of ${n,m,q}$ and can be determined using the best known algorithm for solving LWE. The second is related to the desired upper bound $L$ for the probability of success for an impersonation after $r$ rounds of protocol execution. It has a direct impact in the communication costs, given that the following condition must be met: $(2/3)^r \leq L$.
